DPMesh: Exploiting Diffusion Prior for Occluded Human Mesh Recovery

The recovery of occluded human meshes presents challenges for current methods due to the difficulty in extracting effective image features under severe occlusion. In this paper, we introduce DPMesh, an innovative framework for occluded human mesh recovery that capitalizes on the profound diffusion prior about object structure and spatial relationships embedded in a pre-trained text-to-image diffusion model. Unlike previous methods reliant on conventional backbones for vanilla feature extraction, DPMesh seamlessly integrates the pre-trained denoising U-Net with potent knowledge as its image backbone and performs a single-step inference to provide occlusion-aware information. To enhance the perception capability for occluded poses, DPMesh incorporates well-designed guidance via condition injection, which produces effective controls from 2D observations for the denoising U-Net. Furthermore, we explore a dedicated noisy key-point reasoning approach to mitigate disturbances arising from occlusion and crowded scenarios. This strategy fully unleashes the perceptual capability of the diffusion prior, thereby enhancing accuracy. Extensive experiments affirm the efficacy of our framework, as we outperform state-of-the-art methods on both occlusion-specific and standard datasets. The persuasive results underscore its ability to achieve precise and robust 3D human mesh recovery, particularly in challenging scenarios involving occlusion and crowded scenes.

==> rebuttal/abla_occ_2.tex <==
% \begin{wraptable}{r}{5cm}

\begin{table}[h]
\vspace{-15pt}
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\captionsetup{font={scriptsize}}
 \caption{Ablation study on occluded parts}
\vspace{-10pt}
% \hspace{-.24in}
% \large
 \adjustbox{width=1.1\linewidth}
	{
 \begin{tabular}{lcccc} 
	\toprule 
	Settings &MPJPE$\downarrow$ &PA-MPJPE$\downarrow$ &OCC-MPJPE$\downarrow$ &OCC-PA-MPJPE$\downarrow$ \\
    \midrule
        JOTR [27] & 75.7 & 52.2 & 89.2 & 63.5  \\
    \midrule    
        w/o CAM & 73.7 & 50.6  & 89.4 & 61.0  \\
        w/o NKR & 73.9 & 49.9 & 90.1 & 60.6  \\
    \midrule
        \rowcolor{gray}{DPMesh} & \textbf{70.9} &\textbf{48.0} & \textbf{86.2} & \textbf{57.6}  \\
\bottomrule 
\end{tabular}
 }
    \label{tab:rebb_abla}
    \vspace{-11pt}
% \end{wraptable}
\end{table}


==> rebuttal/abla_occmetric.tex <==
\begin{wraptable}{r}{5cm}
\vspace{-15pt}
% \begin{table}[h]
\small
\setlength{\tabcolsep}{1.5pt}
\captionsetup{font={scriptsize}}
 \caption{Ablation study on occluded parts}
\vspace{-10pt}
\hspace{-.24in}
% \large
 \adjustbox{width=1.1\linewidth}
	{
 \begin{tabular}{lcccc} 
	\toprule 
	Settings &MPJPE$\downarrow$ &PA-MPJPE$\downarrow$ &OCC-MPJPE$\downarrow$ &OCC-PA-MPJPE$\downarrow$ \\
     \midrule
        JOTR [27] & 75.7 & 52.2 & 89.2 & 63.5  \\
    \midrule
        w/o CAM & 73.7 & 50.6  & 89.4 & 61.0  \\
        w/o NKR & 73.9 & 49.9 & 91.1 & 61.6  \\
    \midrule
        \rowcolor{gray}{DPMesh} & \textbf{70.9} &\textbf{48.0} & \textbf{86.2} & \textbf{57.6}  \\
\bottomrule 
\end{tabular}
 }
    \label{tab:rebb_abla}
    \vspace{-11pt}
\end{wraptable}
% \end{table}


==> rebuttal/cross_attn.tex <==
% \vspace{-10pt}
\begin{figure}[!h]
\vspace{-10pt}
  \centering
  %\setlength{\abovecaptionskip}{0cm}
  \includegraphics[width=0.99\linewidth]{rebuttal/cross_attn_2.pdf}
    \vspace{-10pt}
    % \caption{Visualization of the cross-attention map.}
  \label{fig:rebb_cam}
  \vspace{-12pt}
\end{figure}
% \vspace{-10pt}

==> rebuttal/nkr.tex <==
% \vspace{-10pt}
\begin{figure}[!h]
\vspace{-10pt}
  \centering
  %\setlength{\abovecaptionskip}{0cm}
  \includegraphics[width=\linewidth]{rebuttal/inacc2d_2.pdf}
  \vspace{-10pt}
    % \caption{Visualization of the NKR module.}
  \label{fig:rebb_nkr}
  \vspace{-17pt}
\end{figure}
% \vspace{-10pt}

==> rebuttal/sota_comp.tex <==
% \vspace{-10pt}
\begin{wraptable}{r}{4.5cm}
\vspace{-10pt} 
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\captionsetup{font={scriptsize}}
 \caption{\centering{Comparisons on 3DPW}}
\vspace{-10pt}
\hspace{-.28in}
 % \adjustbox{width=1.2\linewidth}
	% {
 \begin{tabular}{lcc} 
	\toprule 
	Method & MPJPE$\downarrow$ &PA-MPJPE$\downarrow$\\
    \midrule
        % FastMETRO (ECCV'22) & 73.5 & 44.6  \\
        HyBrIK  & 71.6 & 41.8 \\
        NIKI  & 71.3 & \textcolor{red}{40.6}  \\
        CLIFF  & 69.0 & 43.0  \\
        % VirtualMarker (CVPR'23) & \textcolor{red}{67.5} & \textcolor{blue}{41.3}  \\
    \midrule
        JOTR &  76.4 & 48.7 \\
        DPMesh & 73.6 & 47.4 \\
    \midrule
        \rowcolor{gray}{DPMesh-ft}  &\textcolor{blue}{68.4} & 42.8  \\
\bottomrule 
\end{tabular}
 % }
    \label{tab:rebb_sota}
\vspace{-10pt} 
\end{wraptable}
% \end{table}
% \vspace{-10pt}

==> rebuttal/sota_comp_2.tex <==
% \vspace{-10pt}
\begin{wraptable}{r}{5cm}
\vspace{-10pt} 
% \centering
\scriptsize
\renewcommand\arraystretch{0.65}
\setlength{\tabcolsep}{1.52pt}
% \captionsetup{font={scriptsize}}
%  \caption{\centering{Comparison with more SOTA methods}}
% \vspace{-10pt}
\hspace{-.2in}
 \adjustbox{width=1.1\linewidth}
	{
 \begin{tabular}{lcccc} 
	\toprule 
	\multirow{2}{*}{Method}& \multicolumn{2}{c}{3DPW} &\multicolumn{2}{c}{3DPW-OC}\\
 \cmidrule(lr){2-3}\cmidrule(lr){4-5}
    &MPJPE$\downarrow$ &PA-MPJPE$\downarrow$  &MPJPE$\downarrow$ &PA-MPJPE$\downarrow$ \\
    \midrule
        % FastMETRO (ECCV'22) & 73.5 & 44.6  \\
        HyBrIK  & 71.6 & {41.8} & 90.8 & 58.8\\
        NIKI  & 71.3 & \textbf{40.6} & 85.5 & 53.5\\
        % CLIFF  & 69.0 & 43.0  \\
        % VirtualMarker (CVPR'23) & \textcolor{red}{67.5} & \textcolor{blue}{41.3}  \\
    % \midrule
    %     JOTR &  76.4 & 48.7 &75.7 &52.2\\
    %     DPMesh & 73.6 & 47.4 & \textbf{70.9}  & \textbf{48.0} \\
    %\textcolor{green!60!black}{(-5.2)} \textcolor{green!60!black}{(-4.6)}
    \midrule
        \rowcolor{gray}{DPMesh-ft}  &\textbf{68.4} & 42.8%41.6
        & \textbf{70.9}  & \textbf{48.0}\\
\bottomrule 
\end{tabular}
 }
    \label{tab:rebb_sota}
\vspace{-15pt} 
\end{wraptable}
% \end{table}
% \vspace{-10pt}
